Bank distress in the news: Describing events through deep learning

While many models are purposed for detecting the occurrence of significant events in financial systems, the task of providing qualitative detail on the developments is not usually as well automated. We present a deep learning approach for detecting relevant discussion in text and extracting natural language descriptions of events. Supervised by only a small set of event information, comprising entity names and dates, the model is leveraged by unsupervised learning of semantic vector representations on extensive text data. We demonstrate applicability to the study of financial risk based on news (6.6M articles), particularly bank distress and government interventions (243 events), where indices can signal the level of bank-stress-related reporting at the entity level, or aggregated at national or European level, while being coupled with explanations. Thus, we exemplify how text, as timely, widely available and descriptive data, can serve as a useful complementary source of information for financial and systemic risk analytics.

==> neurocomp_v0.1.tex <==
\section{Introduction}
\setlength{\parskip}{0.01em}

Text analytics presents both major opportunities and challenges. On the one hand, text data is rich in information and can be harnessed in traditional ways such as for prediction tasks, while its descriptive depth also supports qualitative and exploratory, yet highly data-driven, analysis. On the other hand, decoding and utilizing the expressive detail of human language is prohibitively difficult. In computational terms, text consists of high-dimensional and often ambiguous symbolic input (words), the semantics of which is a product of complex interactions between parts of the sequences in which they occur (phrases, sentences, paragraphs etc.). Text is referred to as sparse data due to the high variability relative to number of samples, and unstructured data as the underlying linguistic structure must be inferred from the surface form as part of the analysis process.

We recognize that many applications of text analytics use linguistically rather na\"ive methods, typically disregarding word order and operating at the symbolic word-level alone. While these applications generally constitute pioneering work in their respective areas, there is currently ample opportunity for advancement, in particular in the intersection between machine learning, computational linguistics and economics. Following the deep learning paradigm, recent developments in natural language processing open up for highly data-driven but linguistically more aware analysis methods, which can be easily applied to new domains and tasks. In this paper, we show how such an approach can be applied to the study of risks in the financial system, with relatively little effort required in terms of collecting data for supervision in new tasks. The method we put forward, applied to bank distress, can provide an index over stress-related reporting in news over time, and retrieve descriptions of the events based on it.

%The global financial crisis has triggered a large number of regulatory
%innovations, yet little progress has occurred with respect to timely
%information on bank vulnerability and risk. This paper provides a
%text-based approach for identifying and describing bank distress using
%news.

Prediction of bank distress has been a major topic both before and following the global financial crisis. Many efforts are concerned with identifying the
build-up of risk at early stages, oftentimes relying upon aggregated
accounting data to measure imbalances (e.g., \cite{cole_predicting_1998,mannasoo_explaining_2009,betz2014predicting}).
Despite their rich information content, accounting data pose two major
challenges: low reporting frequency and long publication lags. A more
timely source of information is the use of market data to indicate
imbalances, stress and volatility (e.g., \cite{Groppetal2006,milne2014}).
Yet, market prices provide little or no descriptive information per
se, and only yield information about listed companies or companies'
traded instruments (such as Credit Default Swaps). This points to
the potential value of text as a source for understanding bank distress. More generally, central banks are starting to recognize the utility of text data in financial risk analytics, too. \cite{riksbank2015bigdata,boe2015textmining}


The literature on text-based computational methods for measuring risk
or distress is still rather scant. For instance, Nyman et al. \cite{Gregoryetal2014}
analyze sentiment trends in news narratives in terms of excitement/anxiety
and find increased consensus to reflect pre-crisis market exuberance,
while Soo \cite{soo2013quantifying} analyses the connection between
sentiment in news and the housing market. Both rely on manually-crafted
dictionaries of sentiment-bearing words. While such analysis can provide
interesting insight as early work on processing expressions in
text to study risk, the approach is generally limiting as dictionaries are cumbersome
to adapt to specific tasks, incomplete and unable to handle semantics beyond single words well. Nevertheless, sentiment analysis based on such simple approaches works quite well due to the fact that it relies on human emotions as strong priors in a way that generalizes across tasks and data, and because lower recall may be countered by the scale of the data. Malo et al. \cite{malo2014good} explore a linguistically more sophisticated approach that models financial sentiment compositionally, although without semantic generalization, supervised by a custom data set of annotated phrases.

Data-driven approaches, such as Wang \& Hua \cite{wang2014copula}
predicting volatility of company stocks from earning calls, may avoid
the issues of handcrafted features and manually annotated corpora. Their method, although allegedly providing good predictive
performance gains, offers only limited insight into the risk-related
language of the underlying text data. It also leaves room for further
improvements with regards to the semantic modeling of individual words
and sequences of words, which we address. Further, Lischinsky \cite{lischinsky2011discourse}
performs a crisis-related discourse analysis of corporate annual reports
using standard corpus-linguistic tools, including some data-driven
methods that enable exploration based on a few seed words. His analysis
focuses extensively on individual words and their qualitative interpretation
as part of a crisis discourse. Finally, R\"onnqvist \& Sarlin \cite{RonnqvistSarlin2015}
construct network models of bank interrelations based on co-occurrence
in news, and assess the information centrality of individual banks
with regards to the surrounding banking system, a fully data-driven approach that could be further enhanced by semantic modeling and conditioning.

We focus on a purely data-driven approach to detect and describe risk, 
in terms of quantitative indices and
extracted descriptions of relevant events. In particular, we demonstrate
this by learning to predict coinciding bank stress based on news,
where a central challenge is to link the sparse and unstructured text
to a small set of reference events. To this end, we demonstrate a
deep learning setup that learns semantic representations of text data
for a predictive model. We train the model to provide coinciding indices
of distress reporting, while, most importantly, connecting text and distress
to provide descriptions. These text descriptions help explain the
quantitative response of the predictive model and allow insight into
the modeled phenomenon. The method is readily adaptable to any phenomenon
by selecting the type of reference events for training.

In the following section, we discuss the text and event data we model on and use to demonstrate
the applicability of our approach to the study of stress. The deep learning setup, including
semantic modeling, predictive modeling and evaluation, extraction of descriptions
and the related indices is explained in Section 3. Finally, we
report our experiments with bank stress data and reflect on the results in Section 4.


\section{Event and text data}

The modeling in our setup is founded on connecting two types of data,
text and event data, by chronology and entities. An event data set contains information on dates and names of involved entities, relating to the specific type of event to be modeled.
Hence, a particular event is first associated with specific text documents using the date and positions in them based on occurrences of the entity name. The model will then learn to generalize across examples and more specifically associate specific language with the target event type.

For the particular study in this paper, the event data set
covers data on large European banks as entities, spanning periods before,
during and after the global financial crisis of 2007--2009. We include
101 banks for which 243 distress events have been observed during 2007Q3--2012Q2.
Following Betz et al. \cite{betz2014predicting}, the events include
government interventions and state aid, as well as direct failures
and distressed mergers. In addition, we map each bank to the country or countries where it is registered, to allow for aggregation of results to the country level.

The text data consist of news articles from Reuters online archive
from the years 2007 to 2014 (Q3). The data set includes 6.6M articles
(3.4B words). 
%As a first step towards linking bank distress events
%and relevant news reporting, we identify mentions of the target banks.
Bank name occurrences are located using a set of patterns defined
as regular expressions that cover common spelling variations and abbreviations.
The patterns have been iteratively developed against the data to increase
accuracy, with the priority of avoiding false positives (in accordance
to \cite{RonnqvistSarlin2015}). Scanning the corpus, 262k articles
are found to mention any of the 101 target banks.

Each article containing matches is cross-referenced against the event data in
order to cast the article as coinciding or not, i.e., likely to discuss the event or not. 
The labeling as coinciding is based on a time window around the event date that the article's date of publication should fall within. An outer time window defines articles published outside as non-coinciding, whereas intermediate articles are discarded to avoid ambiguity. 
We set the inner time window from 8 days before to 45 days after the event, and the outer from 120 days before to 120 days after, as optimized through the evaluation scheme discussed in
Section 3.2.

The training data is organized as tuples of bank name, article and occurrence position (e.g., sentence number), publication date
and the assigned label. The data points are later aggregated monthly and by entity for evaluation of the predictive model and the analysis of distress levels over time.


\section{The semantic deep learning setup}

Characterized in part by the deep, many-layered neural networks, a
prevailing idea of the deep learning paradigm is that machine learning
systems can become more accurate and flexible when we allow for abstract
representations of data to be successively learned, rather than handcrafted
through classical feature engineering. By modeling the input data before modeling specific tasks, the networks can learn about regularities in the world and generalize over them, which improves performance on supervised task learning.
For a recent general survey
on deep learning confer Schmidhuber \cite{schmidhuber2015deep}, and
for a more explicit discussion of deep learning in natural language
processing see Socher \& Manning \cite{manning2013deeplearning}.

While manually designed features help bring structure to the learning
task through the knowledge they encode, they often suffer problems
of being over-specified, incomplete and laborious to develop. Especially
regarding natural language processing, this limits the robustness
of text mining systems and their ability to generalize across languages, domains and
tasks. By exploiting statistical properties of the data,
features can be learned in an unsupervised fashion instead, which
allows for large-scale training not limited by the scarcity of annotated
data. Such intensively data-driven, deep learning approaches have
in recent years led to numerous breakthroughs in application
domains such as computer vision and natural language processing, where
a common theme is the use of unsupervised pre-training to effectively
support supervised learning of deep networks \cite{schmidhuber2015deep}.
We apply the same idea in modeling events in text, as discussed
in the following.


\subsection{Modeling}

We are interested in modeling the semantics of words and compositionality of sequences of words to obtain suitable representations of the content of the news, to use as features for predicting events and associating text descriptions.
At the word level, distributional semantics exploits the linguistic
property that words of similar meaning tend to occur in similar contexts
\cite{harris1954distributional}. Word contexts are modeled to yield
distributed representations of word semantics as vectors, as opposed to declarative formats, which allow
measuring of semantic similarities and detecting analogies without
supervision, given substantial amounts of text \cite{Schutze:1992:DM:147877.148132,schutzePedersen1995irwordsenses,mikolov2013efficient}.
The distributional semantic modeling captures the nature of words in a broader sense, in the directions of syntax and pragmatics.
These word vectors provide an embedding into a continuous semantic space where
the symbolic input of words can be geometrically related to each other,
thus supporting both the predictive modeling in this paper and a multitude
of other natural language processing tasks (e.g., tagging, parsing
and relation extraction \cite{manning2013deeplearning}). 


While traditionally modeled by counting of context words, predictive
models have eventually taken the lead in terms of performance
\cite{baroni2014don}. Neural network language models in particular
have proved useful for semantic modeling, and are especially practical
to incorporate into deep learning setups due to their dense vectors
and the unified neural framework for learning. Mikolov et al. \cite{mikolov2013efficient}
have put forward an efficient neural method that can learn highly
accurate word vectors as it can train on massive data sets in practical
time (a billion words in the order of a day on standard architecture).


\begin{figure}
\begin{center}
\includegraphics[width=0.7\columnwidth]{deepsetup5}
\end{center}
\protect\caption{Deep neural network setup for (a) pre-training of semantic vectors, and
(b) supervised training against event signal $e$.}
\label{fig_deep_setup}
\end{figure}



Subsequently, Le \& Mikolov \cite{le2014distributed} extended the
model in order to represent compositional semantics (cf. \cite{mitchell2010composition})
of sequences of words, from sentences to the length of documents,
which they demonstrated to provide state-of-the-art performance on
sentiment analysis of movie reviews. Methods based on other neural architectures and explicit sentence structure have since gained slightly improved performance \cite{irsoy2014deep,tai2015improved}, but require parse trees as pre-structured input and are therefore not as flexible. Analogous to the sentiment analysis task, we employ
the distributed memory method of Le \& Mikolov to learn vectors for sentences in news
articles, where entities are mentioned, and use them for learning to predict the probability of an event. Hence, when providing bank distress events, the task can be understood as a type of risk sentiment analysis that models language specific to the type of event, rather than more general expression of emotions explicitly.

Our deep neural network for predicting events from text, outlined
in Fig.~\ref{fig_deep_setup}, is trained in two steps: through learning
of sentence vectors as pre-training (\ref{fig_deep_setup}a), followed
by supervised learning against the event signal (\ref{fig_deep_setup}b).
The use of the distributed memory model in the first step is explained
in the following.

The modeling of word-level semantics works by running a sliding window over text, taking a sequence of
words as input and learning to predict the next word (e.g., the 8\textsuperscript{th}
in a sequence), using a feed-forward topology where a projection layer
in the middle provides the semantic vectors once the connection weights have been
learned. A semantic vector $V_i$ is the fixed-length, real-valued pattern of activations reaching the projection layer for network input $i$. The projection layer provides a linear combination that enables
efficient training on large data sets, which is important in achieving
accurate semantic vectors. In addition, the procedure of \cite{le2014distributed} for sentence vector training includes the
sentence ID as input, functioning as a memory for the model that allows
the vector to capture the semantics of continuous sequences rather
than only single words; the sentence ID in fact can be thought of as
an extra word representing the sentence as global context and informing the prediction
of the next word. While the prediction from word context to word constitutes a basic neural language model, the sentence ID conditions the model on the sentence and forces the sentence vector to capture the semantics that is particular to the sentence rather than the language overall. Formally, the pre-training step seeks to maximize
the average log probability:

\[
\frac{1}{t-n}\sum_{i=1}^{t-n}\mathrm{log}\, p(w_{i+n+1}|s,w_{i},...,w_{i+n})
\]
over the sequence of training words $w_{1},w_{2},...,w_{t}$ in sentence
$s$ with word context size $n$. In the neural network, an efficient
binary Huffman coding is used to map sentence IDs and words (an index $i$) to activation patterns in the
input layer, which imposes a basic organization of words by frequency. The illustrated parallel connections are element-wise averaged together as they reach the projection layer.

The second modeling step (Fig. \ref{fig_deep_setup}b) is a normal
feed-forward network fed by the sentence vectors $V_{s}$ (pertaining
to the set of sentences $S$), which we train by Nesterov's Accelerated Gradient \cite{nesterov1983nag} to predict
distress events $e\in\left\{ 0,1\right\}$. Hence, the objective is to maximize the average
log probability:

\[
\frac{1}{|S|}\sum_{s\in S}\mathrm{log}\, p(e_{s}|V_{s})
\]

The network has two output nodes for $e\in\{0,1\}$ in a softmax layer that applies a cross-entropy loss function. In the trained network, the posterior probability $p(e_{d}=1|V_{s})$ reflects the relevance of sentence $s$ to the modeled event type.

Text sequences are also commonly modeled by recurrent neural networks, but are not as efficient as feed-forward topologies with fixed context size.
Compared to sequential text, the sentence vector is a practical fixed-size
representation suitable as input to a feed-forward network. For each
word, the input text originally has a dimensionality equal to the
vocabulary size (typically in the order of a million words), but the semantic modeling
provides reduction to the size of the vector (typically 50--1000).
Both these aspects help train the model against a signal
corresponding to a comparatively tiny number of events. 
In our experiments,
sentence vectors are learned for all entity-mentioning sentences and
the predictive network is trained on individual pairs of sentence
vector and binary event signal, matched together based on date
and entity name occurrence as discussed in Section 2. While this matching procedure furthers the predictive modeling by expanding the example set, compared to the original event data set, the semantic modeling provides necessary generalization of word semantics and representation of compositional semantics.

\subsection{Evaluation and aggregation}

Assuming that the distribution of events for a particular entity is sparse over time, the procedure for matching events to text produces examples with skewed class frequencies. Moreover, it is likely that the user has an imbalanced preference between types of errors, preferring a sensitive system to detect possible events and provide means for further investigation in the form of descriptions, rather than missing an event. This requires extra care in evaluation.

We evaluate the performance of the predictive model to guide hyperparameter optimization and asses the quality of indices that it will produce, and importantly to provide a quantitative quality assurance for the information content of the descriptions
we extract. We use the relative Usefulness measure ($U_{r}$) by Sarlin
\cite{Sarlin2013b}, as it is commonly used in distress prediction
and intuitively incorporates both error type preference ($\mu$) and
relative performance gain of the model. Based on the combination of
negative/positive observations ($\mathrm{obs}\in\left\{0,1\right\}$) and negative/positive
predictions ($\mathrm{pred}\in\left\{0,1\right\}$), we obtain the cases of true
negative ($TN\equiv obs=0\wedge pred=0$), false negative ($FN\equiv obs=1\wedge pred=0$),
false positive ($FP\equiv obs=0\wedge pred=1$) and true positive
($TP\equiv obs=1\wedge pred=1$), for which we can estimate probabilities
when evaluating our predictive model. Further, we define the baseline
loss $L_{b}$ to be the best guess according to prior probabilities
$p(\mathrm{obs})$ and error preferences $\mu$ (Eq. 1) and the model
loss $L_{m}$ (Eq. 2):

\begin{equation}
L_{b}=\mbox{min}\begin{cases}
\mu\cdot p(\mathrm{obs}=1)\\
(1-\mu)\cdot p(\mathrm{obs}=0)
\end{cases}
\end{equation}


\begin{equation}
L_{m}=\mu\cdot p(FN)+(1-\mu)\cdot p(FP)
\end{equation}

From the loss functions we derive Usefulness in absolute ($U_{a}$) and relative terms ($U_{r}$):

\begin{equation}
U_{r}=\frac{U_{a}}{L_{b}}=\frac{L_{b}-L_{m}}{L_{b}}
\end{equation}


While absolute Usefulness $U_{a}$ measures the gain vis-\`a-vis
the baseline case, relative Usefulness $U_{r}$ relates gain to
that of a perfect model (i.e., Eq. 5 with $L_{m}=0\Rightarrow U_{a}=L_{b}$).
Usefulness functions both as a proxy for benchmarking the model (testing)
and to optimize its hyperparameters (validation). Usefulness can also be related to the in text mining
widely used $F$-score\cite{vanRijsbergen1979} (based on $\mathrm{precision}=p(\mathrm{obs}=1|\mathrm{pred}=1)$
and $\mathrm{recall}=p(\mathrm{pred}=1|\mathrm{obs}=1)$):

\begin{equation}
F_{\beta}=(1+\beta^{2})\cdot\frac{\mbox{precision\ensuremath{\cdot}recall}}{(\beta^{2}\cdot\mbox{precision})+\mbox{recall}}
\end{equation}
which similarly can account for varying preferences by
its $\beta$ parameter, although not gain. The $F_{\beta}$-score
assigns $\beta$ times as much importance to recall as to precision
(i.e., preference for completeness over exactness)\cite{vanRijsbergen1979},
which is analogous to but not directly transferable to the $\mu$
parameter in the Usefulness measure. While the $F$-score is commonly
seen to maximize completeness versus exactness of true positives,
the parameter can also be seen as a priority to minimize false negatives
versus false positives (FN prioritized over FP when $\beta>1$). As
a heuristic, we map the balanced, standard $F_{1}$-score with $\beta=1$
to $U_{r}$ with $\mu=0.5$, and match deviations from these preferences
according to $\beta=\mu/(1-\mu)$.

In order to influence the sensitivity of the model, we may classify by threshold on the positive-class posterior probability: $p(e_{d}=1|V_{s})\geq t$. The threshold is optimized on the validation set with respect to Usefulness at a given preference, and applied to the test set for evaluation. However, evaluating classification at the entity level rather than the level of sentence instances is more suitable to the use case, and likely more robust as the classification combines evidence from multiple observed occurrences in the text. The entity-level classification uses the index defined in Eq. 5 below instead of the direct posterior probability, i.e., according to $I(p,b)\geq t$.

Furthermore, evaluation on the sentence vector level with a randomized set split into train, validation and test set may produce somewhat optimistic results, as specific language related to one particular event can be expected to be shared among several instances. Thus, the evaluation would not truly reflect how well the model can be expected to generalize across events of the same type, including future occurrences. To counter the bias, we sample the cross-validation folds according to a \emph{leave-N-entities-out} strategy (or leave-N-banks-out), based by entity rather than instance, such that discussion about a particular entity is compartmentalized into a single set. In case of very frequent entities that would cause very skewed fold sizes, the instances may be split by period such that the more recent occurrences are placed in the latter set (e.g., test rather than validation set) to minimize possible cross-contamination.

\subsection{Event indices}

The aggregated posterior probabilities form an index to reflect the level of event-related reporting about an entity over time, thereby guiding exploration and extraction of descriptions, while it also serves as the signal that we evaluate against. The entity-level relevance index $I:p\times b\rightarrow[0,1]$ is formalized as:

\begin{equation}
I(p,b)=\frac{1}{|S_{p,b}|}\sum_{s\in S_{p,b}}M(V_{s})
\end{equation}
over the sentences $S_{p,b}$ that mention entity $b$ in period $p$,
where $M(V)=p(e=1|V)$ gives the posterior probability of the trained neural network model.

In order to obtain further overview, it may be motivated to further group entities and aggregate their indices. In the experiments, we first aggregate from sentences to banks, and then from banks to countries to highlight national differences across Europe. The second-level index (or country-level index) is a weighted average, defined as:

\begin{equation}
I'(p,c)=\frac{1}{|B_{c}|}\sum_{b\in B_{c}}I(p,b)\cdot|S_{p,b}|
\end{equation}
where $B_{c}$ is the set of entities in category/country $c$.
Finally, we define a top-level index that summarizes the level of relevant reporting for all modeled entities as a global average of vectors:

\begin{equation}
I''(p)=\frac{1}{|S_{p}|}\sum_{s\in S_{p}}M(V_{s})
\end{equation}
where $S_{p}$ is the set of vectors for all entity-mentioning sentences in period $p$.


%%%%%%

\subsection{Extraction of descriptions}

As the neural network in the second step of the deep setup has been trained and the hyperparameters
optimized by cross-validation, it can be applied to sentence vectors $V$ and the posterior
probability $M(V)$ used as a relevance score with respect to the event type. The indices (Eq. 5 and 6) provide overview over time and can highlight peaks and periods with elevated volumes of event-related discussion, which can be more closely investigated by retrieving descriptions of the underlying events.

Given a specific period and entity or set of entities, the basic principle in retrieving descriptions is to filter and rank pieces of text based on the posterior probability of the predictive model for the corresponding semantic vector. In the current setup, we perform the semantic modeling on the sentence level, which simplifies the process of retrieving relevant and specific passages. The semantic modeling can be applied to any type of textual unit, including complete documents, but that requires additional measures for locating the interesting parts within the broader context. R\"onnqvist and Sarlin \cite{ronnqvist2015detect} explore this by applying the same semantic and predictive model on both documents and words, to weight the relevance of the context and individual words respectively. In current experiments, we found that, while their method works for document vectors that are trained on a larger number of words per vector, it does not work well for sentence vectors as they tend to be less similar to the word vectors of the same model. Overall, the extracts as presented in Section 4 are qualitatively better when produced based on sentence-level modeling.

Sentence vectors are trained only for sentences that mention target entity names, as it would be infeasible in terms of memory to model each sentence separately for a large corpus, and because the direct discussion about the entities is the primary interest. The near context of such sentences however tend to support interpretation and are useful to include in presentation. The semantic model supports inference of vectors for at train-time unseen sentences, although with noisier results. We infer vectors and predict the relevance of the sentences immediately before and after sentences in which entities occur, as there is strong dependency between neighboring sentences and a combined score of the expanded context may produce more robust predictions. The combined score for an excerpt is calculated as:

\begin{equation}
x_{i}=max\begin{cases}
M\left(V_{s_{i}}\right)\\
M\left(\frac{1}{n}\sum_{j=1}^{n}V'_{s_{i-1}}\right)\\
M\left(\frac{1}{n}\sum_{j=1}^{n}V'_{s_{i+1}}\right)
\end{cases}
\end{equation}
which includes one sentence before and after sentence $s_{i}$. $V'$ is a stochastic, inferred vector and $n$ is the number of samples (e.g. 100).

The excerpts are ranked according to the score for presentation and offer a preview of the most prominent event-related discussion, which may be retrieved in full from the individual articles. The experiments that follow demonstrate the utility of the excerpts in highlighting the specific forces that drives the index when applied to model bank distress.


\section{Experiments}

We test the deep neural network setup for modeling event-related language on European bank distress events and news data, in order to demonstrate the value it can bring in helping to identify and understand past, ongoing or mounting events. As input for the first step of training the vectors for all
sentences that mention any of the target banks are used. Corresponding
sentence vectors are learned for each of the 716k sentences (originating from 262k articles), while the whole news corpus of 6.6M articles (3.4B words) is sampled in the training process in multiple iterations. Through the semantic modeling on the target sentences, the sentence vectors capture the semantics
specifically of reporting related to our banks of interest, while other text helps model the semantics of English in news reporting in general. We optimized the sentence vector length to 600 and context size to 5 by cross-validation. We also tested the influence of text sequence lengths, and found that training a vector on multiple sentence achieved slightly worse predictive performance, while vectors trained at sentence and document level were comparable.



\subsection{Predictive modeling and evaluation}

Following the semantic pre-training, we train a predictive neural
network model with 3 layers. The input layer has 600 nodes, corresponding
to the semantic vectors and a two output nodes corresponding to distress/tranquil.
As described in Section 2, a set of tuples are complied as data to
learn a predictive model of distress based on sentences. The set consists
of 368k cases, sentences that occur within the time span of the event data and are categorized as either distress-coinciding or non-coinciding. 9.0\% of the cases are labeled as coinciding following our matching procedure. 



We evaluate the predictive model with the four combinations of sampling method and level of evaluation, discussed in Section 3.2. The baseline evaluation with random sampling at the level of sentence vectors is reported in Table \ref{eval_table1} (left), providing 27.5\% relative Usefulness, i.e., performing significantly better than majority class prediction even with the highly skewed class distributions. By comparison, evaluation at the aggregated bank level (classifying by $I(p,b)$ (Eq. 5) rather than $M(V)$) reduces noise from single sentences and stabilizes prediction, thereby increasing performance to 32.6\% (Table \ref{eval_table1}, center). These results show that the model is effective in linking the relevant pieces of text to the bank distress events, hence, providing a first assurance of the quality of the descriptions we will retrieve. Further, we evaluate based on leave-N-banks-out sampling, i.e., the cross-validation folds of vectors are organized by bank, such that the vectors of banks used for testing are held out of training. While this produces lower Usefulness scores, it is a more realistic estimate of future performance in the context of deploying the model on unseen banks or future data. With vector-level evaluation we reach 8.3\% relative Usefulness (Table \ref{eval_table1}, right), while bank-level aggregation again stabilizes prediction and improves performance to 12.3\% of available Usefulness (Table \ref{eval_table2}).


We find the optimal network (50 rectified linear hidden
nodes), hyperparameters for the NAG training algorithm
to train its weights, and threshold on $M(V)$ or $I(b,p)$ for classifying $e\in\left\{ 0,1\right\}$, after which we evaluate performance by $U_r$ of the optimal model. We trained the network by randomized
5-fold cross validation with one fold for validation and one for
testing, in multiple reshuffles of the data set. The evaluation yielded an area under the ROC
%%% todo: update numbers
curve of 0.712 with a standard deviation $\sigma=0.008$ with random sampling evaluated at vector level, and an area of 0.645 ($\sigma=0.083$) with leave-N-banks-out sampling evaluated at bank level. 


\setlength{\tabcolsep}{0.32cm}
\begin{table}
\centering
\begin{tabular}{ccccccccc}
 & \multicolumn{4}{|c|}{Random sampling} & \multicolumn{2}{c|}{Leave-N-banks-out}\tabularnewline
 & \multicolumn{2}{|c}{Vector-level} & \multicolumn{2}{c|}{Aggregated} & \multicolumn{2}{c|}{Vector-level}\tabularnewline

$\mu$ & $\bar{U}_{r}(\mu)$ & $\sigma_{U}$ & $\bar{U}_{r}(\mu)$ & $\sigma_{U}$ & $\bar{U}_{r}(\mu)$ & $\sigma_{U}$\tabularnewline
\hline 
\hline 
0.1 & -0.004 & 0.004 & -0.022 & 0.029 & -0.013 & 0.013\tabularnewline
0.3 & -0.007 & 0.004 & -0.015 & 0.013 & -0.032 & 0.026\tabularnewline
0.5 & 0.002 & 0.005 & -0.014 & 0.010 & -0.039 & 0.036\tabularnewline
0.6 & 0.013 & 0.007 & -0.015 & 0.012 & -0.038 & 0.039\tabularnewline
0.7 & 0.038 & 0.011 & 0.027 & 0.030 & -0.026 & 0.029\tabularnewline
0.8 & 0.095 & 0.019 & 0.156 & 0.029 & -0.008 & 0.044\tabularnewline
0.85 & 0.157 & 0.026 & 0.260 & 0.030 & 0.025 & 0.048\tabularnewline
0.875 & 0.207 & 0.028 & \textbf{0.326} & 0.030 & 0.039 & 0.133\tabularnewline
0.9 & \textbf{0.275} & 0.054 & 0.268 & 0.031 & \textbf{0.083} & 0.114\tabularnewline
0.925 & 0.253 & 0.041 & 0.148 & 0.040 & 0.040 & 0.109\tabularnewline
0.95 & 0.106 & 0.044 & -0.009 & 0.038 & -0.052 & 0.153\tabularnewline
\tabularnewline
\end{tabular}
\\
\protect\caption{Cross-validated predictive performance as relative Usefulness over
preferences between types of error ($\mu$), evaluated at vector and aggregated bank level with random sampling, and at vector level with leave-N-banks-out sampling.}
\label{eval_table1}
\end{table}


\setlength{\tabcolsep}{0.32cm}
\begin{table}
\centering
\begin{tabular}{ccccccccc}
 & \multicolumn{8}{|c|}{Leave-N-banks-out, aggregated}\tabularnewline
$\mu$ & $\bar{U}_{r}(\mu)$ & $\sigma_{U}$ & $\bar{F}_{\beta}$ & $\sigma_{F}$ & $\bar{T\! N}$ & $\bar{F\! N}$ & $\bar{F\! P}$ & $\bar{T\! P}$\tabularnewline
\hline 
\hline 
0.1 & -0.014 & 0.042 & 0.497 & 0.000 & 516 & 68 & 0 & 0\tabularnewline
0.3 & -0.011 & 0.022 & 0.087 & 0.015 & 516 & 68 & 0 & 0\tabularnewline
0.5 & -0.015 & 0.029 & 0.031 & 0.013 & 516 & 68 & 0 & 0\tabularnewline
0.6 & -0.013 & 0.027 & 0.032 & 0.020 & 515 & 68 & 1 & 0\tabularnewline
0.7 & -0.003 & 0.038 & 0.087 & 0.063 & 511 & 65 & 4 & 3\tabularnewline
0.8 & 0.048 & 0.154 & 0.314 & 0.171 & 472 & 53 & 44 & 15\tabularnewline
0.85 & 0.122 & 0.147 & 0.434 & 0.153 & 435 & 45 & 80 & 22\tabularnewline
0.875 & \textbf{0.123} & 0.173 & 0.529 & 0.174 & 374 & 38 & 142 & 30\tabularnewline
0.9 & 0.081 & 0.162 & 0.629 & 0.189 & 308 & 31 & 208 & 37\tabularnewline
0.925 & -0.006 & 0.173 & 0.741 & 0.190 & 151 & 14 & 364 & 54\tabularnewline
0.95 & -0.075 & 0.160 & 0.901 & 0.125 & 38 & 4 & 477 & 64\tabularnewline
\tabularnewline
\end{tabular}
\\
\protect\caption{Cross-validated predictive performance as relative Usefulness and $F$-score over
preferences between types of error ($\mu$) and recall/precision ($\beta$), evaluated at bank level with leave-N-banks-out sampling. Mean confusion matrix values are included, too.}
\label{eval_table2}
\end{table}



Following previous studies \cite{betz2014predicting,Peltonenetal2015}, we make
use of a skewed preference $\mu\approx0.9$ (i.e., missing a crisis is about 9
times worse than falsely signaling one). From the viewpoint of policy,
highly skewed preferences are particularly motivated when a signal
leads to an internal investigation, and reputation loss or other political
effects of false alarms need not be accounted for. We conclude that
at $\mu=0.9$ with vector-level evaluation and at $\mu=0.875$ with aggregated evaluation the model has decent predictive performance by capturing up to
33\% of available Usefulness and 12\% in the more conservative leave-N-banks-out sampled exercise (cf. \cite{betz2014predicting,Peltonenetal2015} for comparable results).
While the model is not robust to low levels of $\mu$, we can see
in Table \ref{eval_table2} that Usefulness is positive and peaking for $\mu$
near 0.9. Meanwhile, $F$-score is reaching its maximum at the extreme preference, which is an indication of its failure to capture gain over the majority class baseline.








\subsection{A descriptive stress index for Europe}

Having trained the network and evaluated its predictive performance,
we can reliably extract descriptive indices of stress at the different levels of aggregation. First, Figure \ref{fig_raw} provides an overview of the raw distress reporting in Europe over the recent years, in terms of distributions of posterior probabilities of the sentence vectors, illustrated through their percentiles. At the same time, this distribution communicates the dynamics of the stress situation in Europe, while the mean (index $I''$ of Eq. 7) summarizes the general trends. 

The time span July 2007 to June 2012 is covered by the event data, and the rest is produced by applying the trained model.
The indices show a sharp double peak starting September 2008, which coincides with the outbreak of the financial crisis. Prior to the most significant peaks, one can also observe elevated values for the indices between August and October 2007, pointing to early discussion on the significance of subprime activities overall and liquidity in European banks. The outbreak of the financial crisis in 2008 is followed by over a year of relatively high stress, where a substantial part of the cross section is elevated. A second significant and similar peak of the stress index is reached in October 2009. At the end of 2010 and 2011, one can observe notable jumps in the most extreme percentiles, whereas the rest of the cross section remains largely unaffected. 






At a general level, the peak in September 2008 can be seen to relate to the overall distress in financial markets due to the collapse of Lehman Brothers in mid-September. However, the fact that values at the top of the distribution appear rather unstable from month to month reflects that different banks are being mentioned over time and usually not persistently across months in distress contexts. By observing increases and peaks in the index of an individual bank or banks in a country, we can locate events of possible relevance to distress. The ability to extract descriptions for these events then becomes useful in order to discern what has happened in relation to banks and distress. Based upon the method described in Section 3.4, these peaks can be described in more detail by extracting top ranking distress-related excerpts. While the overview over Europe supports such analysis, a breakdown into countries or banks brings more distinct patterns forward and allow for deeper and better targeted qualitative analysis. The following section continues the analysis at the country level.



\begin{landscape}
\begin{figure*}
\includegraphics[width=1.5\textwidth]{vector_probabilities}

\protect\caption{Raw distress reporting. Distribution of posterior probabilities over time for sentence vectors, indicating the levels of news reporting relating to bank stress. The blue line indicates
mean, faded lines every 2nd percentile, and dotted lines predictions outside the event sample.}

\label{fig_raw}
\end{figure*}
\end{landscape}




\subsection{Country-level stress, descriptions and interpretation}

From the general stress index for Europe, this section moves to a more granular perspective on stress. We measure stress-related discourse for countries for a more targeted stress measure, which also allows more economic interpretation of developments. Thus, we now aggregate posterior probabilities over time for sentence vectors, indicating the levels of news reporting relating to bank stress, but selectively at a country level (according to Eq. 6). Figure \ref{fig_excerpts1} show the development in stress-related discussion for Belgium and Ireland and Figure \ref{fig_excerpts2} for Germany and UK. The figures illustrate stress levels as time series, as well as annotate peaks of distress levels with top-ranked excerpts. In the appendix, we include plots in Figures \ref{fig_all_index1} and \ref{fig_all_index2} for the other countries whose banks we model.
%, as well as the full versions of the excerpts included in Figures \ref{fig_excerpts1} and \ref{fig_excerpts2}.


\begin{figure*}
\includegraphics[width=0.99\textwidth]{countries_sep_events_excerpts_left}
\protect\caption{Distress index for Belgium and Ireland, with key periods marked and informative excerpts selected from the top-10 of each period and country. Vertical lines indicate distress events and dotted lines out-of-sample predictions. Quotes are from Reuters at given dates.}


\label{fig_excerpts1}
\end{figure*}

\begin{figure*}
\includegraphics[width=0.99\textwidth]{countries_sep_events_excerpts_right}
\protect\caption{Distress index for Germany and United Kingdom, with key periods marked and informative excerpts selected from the top-10 of each period and country. Vertical lines indicate distress events and dotted lines out-of-sample predictions. Quotes are from Reuters at given dates.}


\label{fig_excerpts2}
\end{figure*}




In Figure \ref{fig_excerpts1}, the stress levels for Belgium peak in September 2008. Looking at top-ranked excerpts, September 27 is coupled with a range of rumours in media, yet no official release or actions to mitigate the weakened position of particularly Fortis Bank. Then, the next days we see a bailout of Fortis being discussed as the Belgian, Dutch and Luxembourg governments rescued Fortis. Likewise, the lower chart for Ireland in Figure \ref{fig_excerpts1} shows increased concerns over Bank of Ireland and other large Irish banks in November 2008, as both their earnings and shares were significantly falling. After a range of actions by the state, distress levels were still peaking in September 2009, which is particularly related to the amounts that Allied Irish Banks was putting into the Irish "bad bank". Still, in March 2010 three large Irish banks were still transferring large loans to the National Asset Management Agency (NAMA). Thereafter the most acute stress decreased and has since been at lower levels, although remaining somewhat volatile.

Figure \ref{fig_excerpts2} provides similar stress time series and top-ranked excerpts, but for Germany and UK. Germany can be seen to signal already in August 2007, when IKB's problems were highlighted to potentially lead to "Germany's worst financial crisis in more than 75 years". Three days after this news Deutsche Bank cut a credit line to IKB, as they were worried about IKB's subprime exposures, which further triggered distress in the German banking sector. One reason to the failure of IKB related to an offshore portfolio that was kept off IKB's balance sheet by Rhineland Funding, which is said to have been explained to the largest shareholder KfW. The same large shareholder is then a few months later involved in helping IKB back on its feet with a hefty 4.8 billion euros, as well as additional smaller support afterwards. For UK, stress increased in September 2008, relating not only to previous aid to the UK-based Northern Rock but also to Germany's IKB. Only a few days later in conjunction with a strict clampdown on short-selling, UK-based bank Lloyds Group bought rival HBOS in a rescue takeover. Ironically, a few months later in February 2009 Lloyds in partly nationalized as its HBOS unit made an 8.5 billion pounds loss last year.





\subsection{The case of Fortis and IKB Bank}


This section takes a final step towards more granular output by providing a stress measure for individual banks (according to Eq. 5). As with the country-level aggregates, we can aggregate posterior probabilities for sentence vectors selectively by bank. This output could be derived for each of the 101 banks, yet here we focus on the stress reporting for two banks, namely Fortis and IKB Bank. 

One of the early failures among European financial institutions occurred to the Benelux-based Fortis. As was also highlighted in the above described top distress excerpts for Belgium, Fortis and the rescue procedure was at the core of the discussion in the crisis. We herein focus on the evolution of the distress index for Fortis, as is shown in Figure \ref{fig_single_banks}.
%, and couple excerpts from Fortis-related discussion to the peaks of their distress values. 
To start with, we can observe that elevated values for the stress index coincide with distress events. 


\begin{figure*}
\includegraphics[width=0.99\textwidth]{single_banks}

\protect\caption{Indices (blue) for banks Fortis and IKB indicating the levels of bank stress-related reporting, with faded lines showing every 4th percentile up to the 98th.}


\label{fig_single_banks}
\end{figure*}



By the first event in September 2008, the index rises to 0.30, which marks the start of a prolonged period of elevated stress. The top-ranked excerpts relate to a range of different issues, such as worries about lacking confidence in the markets and the systemic nature of the unfolding crisis:



\begin{quote}\emph{
"Jean-Claude Juncker, also the prime minister of Luxembourg, was asked whether the part nationalisation 
of Dutch-Belgian bank Fortis FOR. -BR and a new injection of liquidity into money markets by the European
 Central Bank would restore market confidence. ``I can only hope that confidence will come back --
  financial markets should not forget to take a close look at the health of fundamental data of several
   banks -- and that this casino game, that's going on independently from the good fundamentals, stops,''
    he told reporters on the sidelines of a meeting in parliament. Belgian, Dutch and Luxembourg
     governments rescued Fortis over the weekend to prevent a domino-like spread of failure by buying its
      shares for 11.2 billion euros."}
(Reuters 2008-09-29, %.2897, 
relevance 0.963, rank 1)
\end{quote}

\begin{quote}\emph{"Investors also worried if a proposed U.S. rescue would stem the contagion that pushed the British government to takeover troubled mortgage lender Bradford \& Bingley BB.L and three European governments to partially nationalize banking and insurance group Fortis FOR.BRFOR.AS."}
(Reuters 2008-09-29, %.2113
relevance 0.923, rank 6)
\end{quote}





%The surge in September 2008 \textbf{???} is more specific in nature. After mentions of Fortis potentially acquiring the insurer Delta Lloyd ABN AMRO Verzekeringen Holding BV, the second excerpt notes that Fortis itself was forced to be nationalized by the Benelux governments in late September. 
In October 2008, the top excerpts discuss the continuing developments such as the Benelux governments "carving up" Fortis to sell to private entities, including French BNP Paribas buying control of the arms in Belgium and Luxembourg. Further excerpts highlight the cross-border aspect of the interventions, and the issues it entails:

\begin{quote}\emph{
"The Fortis deal is the biggest cross-border rescue since the full force of the credit crisis swept across the Atlantic into Europe last month, upending banks and rattling saver confidence."} (Reuters 2008-10-06, %.2483 
relevance 0.945, rank 7)
\end{quote}
\begin{quote}\emph{
"Dutch Finance Minister Wouter Bos fanned Belgian resentment by telling journalists: `Many of the problems were hidden in the Belgian part of the Fortis group.''"} (Reuters 2008-10-05, %.149 
relevance 0.945, rank 8)
\end{quote}

This repeats the message of the already cited news for UK in September 2008, that "there is no consensus on who would bail out a failed multinational bank".


%relate to a divestment of Fortis' Dutch assets in that the Dutch government purchased the banking and insurance divisions in the Netherlands, as well as rumours of Fortis selling its Dutch banking arm to Deutsche Bank. Despite the financial turmoil, a top excerpt shows that the Dutch unit of ABN AMRO that was earlier bought by Fortis showed an increase in profits. 

%As most of the discussion relates to similar issues as at the early stages of the crisis, we only pinpoint a few interesting instances.

%In \textbf{October 2009}, after a number of state interventions, a top excerpt highlights that Deutsche Bank has finally agreed to buy ABN AMRO assets from the Dutch government, which again should enable a merger of the nationalized ABN and Fortis Bank Nederland. 

%Interestingly, while a large number of excerpts still mention various aspects of state interventions, a number of excerpts in \textbf{December 2009} highlight repayment of aid, such as BNP Paribas Fortis repaying a total of 48.8 million euros to Belgium since the guarantees were put in place in May 2009. Likewise, another top-ranked excerpt highlights that BNP Paribas increases its forecast on savings from the integration of former Fortis assets and a successful acquisition of the distressed entity. While being handpicked excerpts of the top ranked excerpts, this provides an idea of how large increases in the built stress index can be accompanied by descriptive excerpts and eventually also the original sources themselves, to help discern the relevant developments in play.

Without a detailed analysis of the discussion around the IKB Bank, we can again conclude from Figure \ref{fig_single_banks} that the stress index takes high values during the realized events. Generally, the top-ranked discussion herein correlates to a large extent with the early top-ranked discussion for Germany, as was above exemplified. The discussion around the distress events relates to early indications of stress, ties to other German banks and government actions taken during and after the stress episodes. After a period of elevated stress during 2007--2008, the figure illustrates that stress is still fairly volatile and that the most extreme percentiles still take large values. This may relate to the fact that discussion keeps relating to the 2007--2008 distress events, in that the solution to the stress events was an acquisition by a investment company. The private equity firm Lone Star acquired IKB Bank in 2008 with the aim of restructuring and selling the bank, and accordingly any rumours still link it to the original stress discussion during the global financial crisis. Such references to past major stress events may however also be an indication of current concerns about financial stress.



\section{Conclusions}

We have presented a deep learning approach that combines two types of data, news text and basic event information, with the aim of linking the two to describe observed and predicted events. The approach entails unsupervised learning on text in order to model its language and provide semantic vector representations that are used as features for predictive modeling of events. The neural network-based method that we put forward is able to work with a very small set of events to discern what type of language and passages in the text are relevant to the modeled event type. The semantic modeling utilizes large amounts of text data to infer abstractions that counter the high variability and sparsity of language, thus supporting prediction of infrequent events. 

The semantic-predictive model can produce indices that indicate the level of relevant discussion over time, overall or related to specific entities or groups thereof. The indices can highlight interesting patterns and offer guidance in the search for relevant events, whereas the model very directly provides means to rank and retrieve pieces of text from the news articles that describe the quantitative signal.

We demonstrate the usefulness of the method and the possibilities of the approach in general within the study of financial risk, by modeling bank distress events. The indices reflect the level of current reporting related to bank stress over time at multiple levels: for Europe in general, individual countries and specific banks. Guided by the indices, users may focus their search and retrieve the relevant reporting of the time, in order to understand the developments regarding, in this case, government interventions and rescues.

The method and our analysis exemplify how text may offer an important complementary source of information for financial and systemic risk analytics, which is readily available, current and rich in descriptive detail. We recognize that deep learning approaches are useful in particular to handle the complexities of such new types of data, while offering necessary flexibility when exploring new fields of analysis. Seeking to harness the expressiveness of text, we should look to computational linguistics for support in terms of theoretical foundations and tools.

While we show that it is possible to predict relevance and retrieve informative descriptions of events, we merely scratch the surface of the vast text material in a cross section with our current method of presentation. A challenge remains in developing methods that are able to meaningfully summarize the broader base that may include a long tail of weakly signaling, subtile expression. Such signals may be particularly important in order to register and track developments before they materialize in severe and obvious events.



\section{Appendix}

%\subsection{Selected top-ranked country excerpts}

%\begin{quote}\emph{
%"As of Saturday, financial authorities were contacting other institutions, a source familiar with the situation told Reuters, although no particular solution was preferred and nothing concrete was likely to emerge before Sunday. Fortis investors face a weekend of uncertainty after the banking and insurance group went out of its way on Friday to reassure them that it was solvent and in no danger of collapse following market talk the company could become another casualty of the credit crisis. Veerle De Schryver, a spokewoman for the Banking, Financial and Insurance Commission (CBFA), said: ``The parties will discuss scenarios for Fortis in a cooperative way.''"} (Reuters 2008-09-27) %.198
%\end{quote}

%\begin{quote}\emph{
%""
%}\end{quote}

%\begin{quote}\emph{}\end{quote}

Figures \ref{fig_all_index1} and \ref{fig_all_index2} provide country-level indices for the countries not included in Figures \ref{fig_excerpts1} and \ref{fig_excerpts2}, as well as the non-weighted average of all country indices.

\begin{figure*}
\includegraphics[width=0.99\textwidth]{countries_all_sep_events1}
\protect\caption{Distress index for Austria, Switzerland, Cyprus, Denmark, Spain, France, Greece and average of all modeled countries. Vertical lines indicate bank-level distress events and dotted lines out-of-sample predictions.}


\label{fig_all_index1}
\end{figure*}

\begin{figure*}
\includegraphics[width=0.99\textwidth]{countries_all_sep_events2}
\protect\caption{Distress index for Hungary, Italy, Luxembourg, Latvia, Netherlands, Portugal, Sweden and Slovenia. Vertical lines indicate bank-level distress events and dotted lines out-of-sample predictions.}


\label{fig_all_index2}
\end{figure*}

